On the Control of Self-Balancing Unicycles

This paper discusses the problem of designing a self-balancing unicycle where pedals are used for both power generation and speed control. After developing the principal physical aspects (in the longitudinal dimension), we describe an abstract model in the form of a collection of hybrid automata, together with design requirements to be met by an ideal controller. We discuss simplifications and assumptions that make this model amenable to verification and validation tools such as SpaceEx. To enable experimentation with different prototypical controllers and user behaviours in concrete scenarios, we also develop a simple simulation framework using digital time.

==> eptcsdata.tex <==
\providecommand{\firstpage}{25}
\providecommand{\publicationstatus}{R.J. van Glabbeek, J.F. Groote \& P. H\"ofner (Eds.):
Workshop on\\
Models for Formal Analysis of Real Systems (MARS 2015)\\
EPTCS 196, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.196.3}{10.4204/EPTCS.196.3}}
\pdfoutput=1

